Stochastic Gradient Descent with Nonlinear Conjugate Gradient-Style Adaptive Momentum

Momentum plays a crucial role in stochastic gradient-based optimization algorithms for accelerating or improving training deep neural networks (DNNs). In deep learning practice, the momentum is usually weighted by a well-calibrated constant. However, tuning hyperparameters for momentum can be a significant computational burden. In this paper, we propose a novel \emph{adaptive momentum} for improving DNNs training; this adaptive momentum, with no momentum related hyperparameter required, is motivated by the nonlinear conjugate gradient (NCG) method. Stochastic gradient descent (SGD) with this new adaptive momentum eliminates the need for the momentum hyperparameter calibration, allows a significantly larger learning rate, accelerates DNN training, and improves final accuracy and robustness of the trained DNNs. For instance, SGD with this adaptive momentum reduces classification errors for training ResNet110 for CIFAR10 and CIFAR100 from $5.25\%$ to $4.64\%$ and $23.75\%$ to $20.03\%$, respectively. Furthermore, SGD with the new adaptive momentum also benefits adversarial training and improves adversarial robustness of the trained DNNs.

==> preamble.tex <==
% ---------------------------------
%floats and figures
% ---------------------------------

% if you need to pass options to natbib, use, e.g.:
\PassOptionsToPackage{numbers, compress}{natbib}
\usepackage{amsmath}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}
\urlstyle{same}
%\usepackage{array}
\usepackage{booktabs} % for professional tables
\usepackage{amsfonts}
\usepackage{bm}
%\usepackage{soul}
%\usepackage{lmodern}
%\usepackage{booktabs}
\usepackage{threeparttable}
%\usepackage{mathtools}
\usepackage{tablefootnote}

%\usepackage{cuted}
\usepackage{lipsum}
\usepackage{comment}

\usepackage{multirow}
\usepackage[usenames, dvipsnames]{color}
\usepackage{amsmath}

\newcommand\xmod[1]{{\textcolor{blue}{#1}}}
\newcommand\zmod[1]{{\textcolor{red}{#1}}}


\usepackage{hyperref}

\usepackage{enumitem}

\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\usepackage{listings}

\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}

\usepackage{listings}
\usepackage{color}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color
  basicstyle=\footnotesize,        % size of fonts used for the code
  breaklines=true,                 % automatic line breaking only at whitespace
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  keywordstyle=\color{blue},       % keyword style
  stringstyle=\color{mymauve},     % string literal style
}

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}
% \usepackage[disable]{todonotes}
% \usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
%takes in optional argument
% \newcommand{\tocite}[1]{%
% \textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
% }


\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

%version in control in draft mode
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
% \newcommand{\figref}[1]{Fig.    \,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
% \newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

\newcommand{\tss}{\hspace*{0.66mm}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{0.5mm}
\setlength{\belowcaptionskip}{0mm} 
\setlength{\textfloatsep}{1.5mm}
\setlength{\dbltextfloatsep}{1.5mm}
%\renewcommand{\baselinestretch}{.9945}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions for equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

